A Low-Rank Approach to Off-The-Grid Sparse Deconvolution

We propose a new solver for the sparse spikes deconvolution problem over the space of Radon measures. A common approach to off-the-grid deconvolution considers semidefinite (SDP) relaxations of the total variation (the total mass of the absolute value of the measure) minimization problem. The direct resolution of this SDP is however intractable for large scale settings, since the problem size grows as $f_c^{2d}$ where $f_c$ is the cutoff frequency of the filter and $d$ the ambient dimension. Our first contribution introduces a penalized formulation of this semidefinite lifting, which has low-rank solutions. Our second contribution is a conditional gradient optimization scheme with non-convex updates. This algorithm leverages both the low-rank and the convolutive structure of the problem, resulting in an $O(f_c^d \log f_c)$ complexity per iteration. Numerical simulations are promising and show that the algorithm converges in exactly $r$ steps, $r$ being the number of Diracs composing the solution.

==> sections/01-preliminaries.tex <==
\section{Preliminaries}
\label{sec::preliminaries}

In this section, we briefly recall some theoretical insight about \eqref{eq:blasso} and its dual. In particular, we introduce the important notion of dual certificate.
%%%%%%%%%%%%%%%%%
\subsection{Total variation norm}
%%%%%%%%%%%%%%%%%

The total variation norm of a measure $\mu \in \Radon{\Torus^d}$ is defined as
\eq{\label{eq:tvnorm}		% TV NORM
	\normtv{\mu}{\Torus^d} \eqdef \sup\enscond{\Re\Big(\int_{\Torus^d} \overline{\eta} \diff \mu\Big)}{\eta \in \Cont{\Torus^d}, \quad \normi{\eta} \leq 1}.
}%
It is the natural extension of the discrete $\lun$-norm to the space of Radon measures. Indeed, if for instance $\mu$ is some discrete measure $\mu = \mu_{a,x} \eqdef \sum a_k \de_{x_k}$, then $\normtv{\mu}{\Torus^d} = \normu{a}$. Similarly, if $\mu$ admits a density $f$ with respect to the Lebesgue measure, then $\normtv{\Torus^d}{\mu} = \norm{f}_1$. The subdifferential of the total variation norm reads
\eql{\label{tv-subdiff}	% TV SUBDIFF
	\partial \normtv{\mu}{\Torus^d} = \enscond{\eta \in \Cont{\Torus^d}}{\normi{\eta} \leq 1, \quad \Re\Big(\int_{\Torus^d} \overline{\eta} \diff \mu\Big) = \normtv{\mu}{\Torus^d}}.
}%
In particular, for a discrete measure, one has
\eq{ 		% TV SUBDIFF DISCRETE MEASURE
	\partial \normtv{\mu_{a,x}}{\Torus^d} = \enscond{\eta \in \Cont{\Torus^d}}{\normi{\eta} \leq 1, \quad \eta(x_k) = \frac{a_k}{\abs{a_k}} \quad k = 1, \ldots, r}.
}%



%%%%%%%%%%%%%%%%%
\subsection{Primal and Dual problems}
\label{subsec::preliminaries}
%%%%%%%%%%%%%%%%%

The dual of the BLASSO reads \cite{tang-recht15,duval15}
\eq{\label{eq:dual}\tag{$\Dd_\la(y)$}	% DUAL BLASSO
	\uargmax{p \in \CC^{n_c}} \Re\dotp{y}{p} - \frac{\la}{2}\norm{p}^2 \quad \text{s.t.} \quad \normi{\Phi\adj p} \leq 1.
}%
where $n_c \eqdef (2f_c+1)^d$. Here the computational challenge comes from the infinite number of constraints, asking for a trigonometric polynomial to be bounded by one in magnitude.



\paragraph{Dual certificate} Strong duality holds between \eqref{eq:blasso} and \eqref{eq:dual} \cite[Proposition 2]{bredies13}, and optimality relations between any pair of solutions $(\mu_\la, p_\la)$ read
\eql{\label{optimality}		% OPTIMALITY RELATIONS
	\left\{
		\begin{array}{lll}
			\Phi\adj p_\la \in \partial\normtv{\mu_\la}{\Torus^d}\\
			p_\la = \frac{1}{\la}(y-\Phi\mu_\la)
		\end{array}
	\right..
}%
The trigonometric polynomial $\eta_\la = \Phi^* p_\la$ is called the \textit{dual certificate} \cite{candes10}. The associated complex polynomial $P_{p_\la}$ is Hermitian.

We now recall some important basic results about the primal and dual solutions, with brief proof so that the paper be self-contained.
%%%PROPOSITION
\begin{prop}\label{prop::support}
Let $\Sigma\left[p\right] = \enscond{x \in \TT^d}{\abs{\Phi\adj p(x)}=1}$. Then $\Supp \mu_\la \subset \Sigma\left[p_\la\right]$.
\end{prop}
\begin{proof} % ----------
%Let $\eta_\la = \Phi^*p_\la$. Writing $\mu_\la = \mu_{\la+} - \mu_{\la-}$, where $\mu_{\la+}$ and $\mu_{\la-}$ are both positive measures, the total variation of $\mu_\la$ can be written $\abs{\mu_\la} = \mu_{\la+} + \mu_{\la-}$. Then, using \eqref{optimality} and \eqref{tv-subdiff}, we obtain
%\eq{  
%	0 = \normtvTd{\mu_\la} - \int \eta_\la \diff\mu_\la = \int_{\TT^d} (1-\eta_\la)\diff\mu_{\la+} + \int_{\TT^d} (1+\eta_\la)\diff\mu_{\la-}.
%}%
%Since $\normi{\eta_\la} \leq 1$, we have $\int (1-\eta_\la)\diff\mu_{\la+} = \int (1+\eta_\la)\diff\mu_{\la-} = 0$. Therefore, $\eta_\la = 1$ $\mu_{\la+}$-a.e. and $\eta_\la = -1$ $\mu_{\la-}$-a.e., which leads to $\abs{\eta_\la} = 1$ $\mu$-p.s.

The polar decomposition lemma for complex measures ensures that there exists a measurable function $\xi: \Torus^d \rightarrow \CC$ such that $\abs{\xi} = 1$ and $\mu = \xi \abs{\mu}$.  Let $\eta_\la = \Phi^*p_\la$. Using \eqref{optimality} and \eqref{tv-subdiff}, we get
\eq{  
	0 = \normtv{\mu_\la}{\Torus^d} - \Re\Big(\int_{\Torus^d} \overline{\eta_\la} \diff \mu_\la\Big) = \int_{\Torus^d} (1-\Re(\overline{\eta_\la}\xi))\diff\abs{\mu_\la}.
}%
Since $\normi{\eta_\la} \leq 1$ and $\abs{\xi(x)}=1$ for all $x \in \Torus^d$, it follows that $1 \geq \Re(\overline{\eta_\la}\xi)$. The equality above thus implies $\Re(\overline{\eta_\la}\xi) = 1$ $\mu_\la$-a.e., which leads to $\abs{\eta_\la} = 1$ $\mu_\la$-a.e. since $1 \geq \abs{\eta_\la}^2 = \abs{\overline{\eta_\la}\xi}^2 \geq \Re(\overline{\eta_\la}\xi)^2$.
\end{proof} % ----------P
The dual polynomial, bounded by one in magnitude, thus interpolates the signs of the spikes on the support of $\mu_\la$, see Fig.~\ref{dual-poly}. One can then recover the measure $\mu_\la$ using the following result.

%%%PROPOSITION
\begin{prop}\label{prop::unicity}
Assume that $\Sigma_\la \eqdef \Sigma\left[p_\la\right]$ is finite. Let $\Phi_{\Sigma_\la}$ be the operator defined as $\Phi_{\Sigma_\la} : a \in \CC^{\abs{\Sigma_\la}} \mapsto \sum_{s \in \Sigma_\la} a_s \Phi(\de_s)$. If $\Phi_{\Sigma_\la}$ is injective, \eqref{eq:blasso} has a unique solution $\mu_ \la$ given by
\eq{
	\mu_\la = \sum_{s \in \Sigma_\la} a_s \de_s, \qwhereq a = (\Phi_{\Sigma_\la}^*\Phi_{\Sigma_\la})^{-1}\Phi_{\Sigma_\la}^*(y-\la p_\la).
}%
\end{prop}
\begin{proof} % ----------
Let $\mu_\la$ and $\mu_\la'$ be solutions of \eqref{eq:blasso}. Using Proposition~\ref{prop::support}, we may write $\mu_\la = \sum_{s \in \Sigma_\la} a_s \de_s$ and $\mu_\la' = \sum_{s \in \Sigma_\la} a_s' \de_s$. Thus
%eq
\eql{\label{linsys}
	\Phi_{\Sigma_\la} a = \Phi \mu_\la = y - \la p_\la = \Phi \mu_\la' = \Phi_{\Sigma_\la} a'
}
%
which implies $a=a'$, and therefore $\mu_\la = \mu_\la'$. Moreover, the previous relation immediately yields $a = (\Phi_{\Sigma_\la}^*\Phi_{\Sigma_\la})^{-1}\Phi_{\Sigma_\la}^*(y-\la p_\la)$.
\end{proof} % ----------P



\paragraph{Support recovery} Finding the support of $\mu_\la$ thus boils down to determining the set $\Sigma_\la$, \ie the points where the dual polynomial $\eta_\la$ saturates the constraint in \eqref{eq:dual}. This is actually equivalent to finding the roots of unit modulus of a certain polynomial. Let $P_\la(z) = 1 - \left| \sum_{k \in \Om_c} p_{\la,k}z^k \right|^2$

%%%PROPOSITION
\begin{prop}\label{prop::rootfinding}
Suppose that the hypothesis of Proposition~\ref{prop::unicity} hold.
Let $\tilde{P}_\la = 1 - \abs{P_{p_\la}}^2$. Then:
\eq{
	 \Supp \mu_\la \subset \frac{1}{2\pi} \arg \enscond{z \in \CC^d}{\tilde{P}_\la(z) = 0 \qandq \abs{z_i}=1, \;\; i = 1, \ldots, d}
}%
\end{prop}
\begin{proof} % ----------
From Proposition~\ref{prop::unicity}, we know that $\supp \mu_\la \subset \Sigma_\la$. Then we have
\eq{
	x \in \Sigma_\la \Leftrightarrow \tilde{P}_\la(e^{2i\pi x}) = 0 \Leftrightarrow x \in \frac{1}{2\pi}\arg \enscond{z \in \CC^d}{\tilde{P}_\la(z) = 0 \qandq \abs{z_i}=1, \;\; i = 1, \ldots, d}
}%
which yields the result.
\end{proof} % ----------P

\begin{rem} Should the inclusion above ever be strict, solving the linear system \eqref{linsys} which gives the amplitudes leads to null amplitudes for points located in $\Sigma_\la \setminus \Supp \mu_\la$, provided $\Phi_{\Sigma_\la}$ injective.
\end{rem}

%%%REMARK
\begin{rem}\label{double-roots} %Since $P_{p_\la}$ is Hermitian, $P_{p_\la}(z) = \overline{P_{p_\la}(1/\bar{z})}$, hence $Q_\la(z) = Q_\la(1/\bar{z})$. Therefore, the roots of $Q_\la$ wich satisfy $\abs{z}=1$ coincide with its double roots. 
For multivariate polynomials, this root-finding problem is very difficult. We discuss our numerical approach further on, see Section~\ref{numerics}.
\end{rem} % ----------R


%%%FIGURE
\begin{figure}
	\includegraphics[width=0.5\textwidth]{figures/dual_polynomial1}
	\includegraphics[width=0.5\textwidth]{figures/dual_polynomial2}
	\caption{\textit{Left}: $d=1$, $f_c = 13$, $r=5$, $\norm{w} = 0$, $\lambda = 5\times10^{-3}$. \textit{Right}: $d=2$, $f_c = 7$, $r=5$, $\norm{w} = 0$, $\lambda = 10^{-2}$. Dual polynomials; true positions of Diracs are shown in red (positive spikes) or cyan (negative spikes).}
	\label{dual-poly}
	\postimagespace
\end{figure} % ----------F















%%%%%%%%%%%%%%%%%%%%
%\subsection{Measures and moments (\textcolor{red}{TODO: REMOVE})}
%Semidefinite formulations arise from theory of moments and theory of positive polynomials. The connection was made by Lasserre.
%
%Define moment matrix, corresponding linear application: $c = (c_\al) \in \CC^{?}$, Moment matrix is the matrix associated with the linear form $L(c): \xi \mapsto \sum_{\al,\be} c_{\al-\be} \xi_\al \bar{\xi}_\be$? $L(c) = \xi \mapsto \sum_{\al} c_\al \xi_\al$?
%\eq{
%	M(c)_{\al,\be} = L(c)(x^\al \bar{x}^\be) = c_{\al-\be}
%}
%%% THEOREM %%
%\begin{thm}[Caratheodory-T\oe plitz]
%(I am not sure this is exactly Caratheodory-Toeplitz theorem in the case of the truncated moment problem, \ie considering only a finite sequence of moments)
%
%For $n \in \NN^*$, given $c = (c_1, \ldots, c_n) \in \CC^{n}$, there exists a positive measure $\mu$ such that
%
%% eq
%\eq{
%	c_k = \frac{1}{2\pi} \int_0^{2\pi} e^{ik\theta} \diff\mu(e^{i\theta}), \quad 0 \leq k \leq n
%}
%%
%if and only if the matrix $M(c) = (c_{j-k})_{0\leq j,k\leq n}$, with $s_{-j} = s_j^*$ is positive semidefinite. Moreover this measure is not unique if and only if $M(c) \succ 0$. 
%\end{thm}
%%%%%%%
%TODO: references to check: \cite{li06, Akhiezer, curto00}
%
%TODO: multivariate case?
%
%Link between measure and moment matrix
%%% THEOREM %%
%\begin{thm}[$\sim$ Theorem 3.11 in \cite{Lasserre}?]
%Let $c = (c_\ga)$ be a finite sequence with $\abs{\ga} \leq 2r$. Then $c$ has a $\rank M(c)$-atomic representing measure $\mu \in \Mm(\TT^d)$ if and only if
%\begin{enumerate}
%	\item $M(c) \succeq 0$,
%	\item $\rank M_r(c) = \rank M_{r-1}(c)$ ????
%\end{enumerate}
%\end{thm}
%%%%%%%



%%%%%%%%%%%%%%%%%%%%%
%\subsection{Trigonometric polynomials (\textcolor{red}{TODO: REMOVE})}
%The theory of positive polynomials is in duality with the theory of moments (linked through convex duality with Schm\"{u}dgen theorem \cite{schmudgen91} in the real case, refined later by Putinar \cite{putinar93} and Jacobi and Prestel \cite{jacobi01}).
%
%%% THEOREM %%
%\begin{thm}[Fej\'{e}r-Riesz]
%A univariate Hermitian trigonometric polynomial $P \in \CC$ is nonnegative on the unit circle if and only if there exists a causal polynomial $H$ such that
%
%% eq
%\eq{
%	P(z) = H(z) H^*(z^{-1})
%} 
%%
%\end{thm}
%%%%%%%
%
%%% THEOREM %%
%\begin{thm}[Positivstellensatz {\cite[Theorem 3.5]{Dumitrescu}} ]
%If a $d$-variate Hermitian trigonometric polynomial is positive on the unit $d$-circle, then it is sum-of-squares. 
%\end{thm}
%%%%%%%
%
%%% LEMMA %%
%\begin{lem}[Bounded Real Lemma {\cite[Corollary 4.25]{Dumitrescu}}] Let $H$ be a positive orthant polynomial (equivalent of causal polynomial in dimension greater than 1). If $\abs{H(\om)} < \ga, \forall \om \in \TT^d$, then there exists a matrix $Q \succeq 0$ such that
%
%% eq
%\eq{
%	\begin{aligned}
%		\ga^2 \de_{\kk}& = \tr \left[ \Theta_{\kk} Q \right], \quad \kk \in \Hh, \\
%		&\begin{bmatrix} Q & h \\ h^* & 1 \end{bmatrix} \succeq 0
%	\end{aligned}
%}
%%
%
%\end{lem}


%%%%%%%%%%%%%%%%
%\subsection{Support recovery}
%\paragraph{From dual}
%Support recovery via root-finding: dual polynomial real-valued trigonometric polynomial, support coincides with roots of real polynomial $1 - \abs{\eta}^2$ that are located on the unit circle.
%
%\paragraph{From primal}
%Vandermonde decomposition
